QAQ: Quality Adaptive Quantization for LLM KV Cache

The emergence of LLMs has ignited a fresh surge of breakthroughs in NLP applications, particularly in domains such as question-answering systems and text generation. As the need for longer context grows, a significant bottleneck in model deployment emerges due to the linear expansion of the Key-Value (KV) cache with the context length. Existing methods primarily rely on various hypotheses, such as sorting the KV cache based on attention scores for replacement or eviction, to compress the KV cache and improve model throughput. However, heuristics used by these strategies may wrongly evict essential KV cache, which can significantly degrade model performance. In this paper, we propose QAQ, a Quality Adaptive Quantization scheme for the KV cache. We theoretically demonstrate that key cache and value cache exhibit distinct sensitivities to quantization, leading to the formulation of separate quantization strategies for their non-uniform quantization. Through the integration of dedicated outlier handling, as well as an improved attention-aware approach, QAQ achieves up to 10x the compression ratio of the KV cache size with a neglectable impact on model performance. QAQ significantly reduces the practical hurdles of deploying LLMs, opening up new possibilities for longer-context applications. The code is available at github.com/ClubieDong/KVCacheQuantization.

==> chapters/old_method.tex <==
\newcommand\paren[1]{\left(#1\right)}
\newcommand\norm[1]{\left\lVert#1\right\rVert}
\newcommand\abs[1]{\left\lvert#1\right\rvert}
\newcommand\ceil[1]{\left\lceil#1\right\rceil}

\section{Quality Adaptive Quantization Method for Key Cache and Value Cache}

\shichen{This is just an edited version of my manuscript, should not be used directly in the final paper.}

\subsection{Notations}

\begin{itemize}
    \item $D$: Size of hidden layer per head.
    \item $d$: Subscription of hidden layer per head, $1\le d\le D$.
    \item $T$: Length of the sequence.
    \item $t$: Subscription of the sequence, $1\le t\le T$.
    \item $\textbf{Q}$: Query tensor with shape $\paren{1,D}$.
    \item $\textbf{K}$: Key tensor with shape $\paren{T,D}$.
    \item $\textbf{V}$: Value tensor with shape $\paren{T,D}$.
    \item $\textbf{A}$: Attention tensor before softmax with shape $\paren{1,T}$.
        $$\textbf{A}=\frac{1}{\sqrt{D}}\cdot\textbf{Q}\cdot\textbf{K}^T$$
    \item $\textbf{S}$: Attention tensor after softmax with shape $\paren{1,T}$.
        $$\textbf{S}=\text{Softmax}\paren{\textbf{A}}$$
    \item $\textbf{X}$: Final result tensor of attention module with shape $\paren{1,D}$.
        $$\textbf{X}=\textbf{S}\cdot\textbf{V}$$
    \item $\hat{\textbf{K}}$, $\hat{\textbf{V}}$, $\hat{\textbf{A}}$, $\hat{\textbf{S}}$, $\hat{\textbf{X}}$: Quantized tensor of $\textbf{K}$, $\textbf{V}$, $\textbf{A}$, $\textbf{S}$, $\textbf{X}$.
    \item $E^{\paren{\textbf{S}}}$, $E^{\paren{\textbf{X}}}$: Mean squared error (MSE) calculated from the quantized tensor $\hat{\textbf{S}}$ and $\hat{\textbf{X}}$.
    \item $E^{\paren{\textbf{S}}}_\text{max}$, $E^{\paren{\textbf{X}}}_\text{max}$: Maximum allowed mean squared error (MSE) of $\hat{\textbf{S}}$ and $\hat{\textbf{X}}$, given as two hyper-parameters.
    \item $\Delta K_t$, $\Delta V_t$: Mean absolute error (MAE) per token of $\hat{\textbf{K}}_t$, $\hat{\textbf{V}}_t$, calculated from $E^{\paren{\textbf{S}}}$ and $E^{\paren{\textbf{X}}}$, respectively.
    \item $B^{\paren{\textbf{K}}}_t$, $B^{\paren{\textbf{V}}}_t$: Number of quantization bits per token of $\textbf{K}_t$ and $\textbf{V}_t$, calculated from $\Delta K_t$ and $\Delta V_t$, respectively.
\end{itemize}

\subsection{Overview}

We split the quantization process into three steps:
\begin{itemize}
    \item \textbf{Step 1}: calculate $\Delta V_t$ using $E^{\paren{\textbf{X}}}$.
    \item \textbf{Step 2}: calculate $\Delta K_t$ using $E^{\paren{\textbf{S}}}$.
    \item \textbf{Step 3}: calculate $B^{\paren{\textbf{K}}}_t$ and $B^{\paren{\textbf{V}}}_t$ using $\Delta K_t$ and $\Delta V_t$, respectively.
\end{itemize}

We call step 1 and step 2 the \emph{attention-aware quantization}, step 3 the \emph{distribution-aware quantization}.

\subsection{Step 1: value cache quantization}

$E^{\paren{\textbf{X}}}$ is calculated as:
\begin{align*}
E^{\paren{\textbf{X}}}
=&\frac{1}{D}\cdot\norm{\hat{\textbf{X}}-\textbf{X}}_2^2
=\frac{1}{D}\cdot\norm{\textbf{S}\cdot\hat{\textbf{V}}-\textbf{S}\cdot\textbf{V}}_2^2\\
\triangleq&\frac{1}{D}\cdot\norm{\textbf{S}\cdot\Delta\textbf{V}}_2^2
=\frac{1}{D}\cdot\sum_{d=1}^D\norm{\textbf{S}\cdot\Delta\textbf{V}_{:,d}}_2^2\\
=&\frac{1}{D}\cdot\sum_{d=1}^D\paren{\sum_{t=1}^TS_t\cdot\Delta V_{t,d}}^2
\end{align*}

Since we would like to equally divide the quantization error into every token and let $\Delta V_{t,d}$ be as small as possible \shichen{Need more argumentation}, we let the following inequality hold for all $d=1,\cdots,D$ and $t=1,\cdots,T$:
$$
E^{\paren{\textbf{X}}}_\text{max}\ge\frac{1}{D}\cdot D\cdot\paren{T\cdot S_t\cdot\Delta V_{t,d}}^2
$$

Therefore, we get:
$$
\Delta V_t=\Delta V_{t,d}\le\frac{\sqrt{E^{\paren{\textbf{X}}}_\text{max}}}{T}\cdot\frac{1}{\lvert S_t\rvert}
$$

\subsection{Step 2: key cache quantization}

$E^{\paren{\textbf{S}}}$ is calculated as:
$$
E^{\paren{\textbf{S}}}
=\frac{1}{T}\cdot\norm{\hat{\textbf{S}}-\textbf{S}}_2^2
=\frac{1}{T}\cdot\sum_{t=1}^T\paren{\hat{S}_t-S_t}^2
$$

We treat $E^{\paren{\textbf{S}}}$ as a function of $\hat{\textbf{K}}$ and Taylor expand it at $\hat{\textbf{K}}=\textbf{K}$ to the second order:
\begin{align*}
E^{\paren{\textbf{S}}}\paren{\hat{\textbf{K}}}
\approx E^{\paren{\textbf{S}}}\paren{\textbf{K}}
&+\nabla E^{\paren{\textbf{S}}}\paren{\textbf{K}}^T\cdot\Delta\textbf{K}\\
&+\frac{1}{2}\cdot\Delta\textbf{K}^T\cdot\textbf{H}\paren{\textbf{K}}\cdot\Delta\textbf{K}
\end{align*}
where $\nabla E^{\paren{\textbf{S}}}\paren{\textbf{K}}$ and $\textbf{H}\paren{\textbf{K}}$ are the gradient and the Hessian matrix of $E^{\paren{\textbf{S}}}$ at $\hat{\textbf{K}}=\textbf{K}$, respectively, $\Delta\textbf{K}$ is defined as $\hat{\textbf{K}}-\textbf{K}$.

Taking the derivative of $E^{\paren{\textbf{S}}}$ with respect to $\hat{\textbf{K}}$ using the chain rule for multi-variable functions, we get:
\begin{align*}
\frac{\partial E^{\paren{\textbf{S}}}}{\partial\hat{K}_{a,b}}
=&\frac{2 Q_b}{\sqrt{D}\cdot T}\sum_{t=1}^T\paren{\hat{S}_t-S_t}\cdot\frac{\partial\hat{S}_t}{\partial\hat{A}_a}\\
\frac{\partial^2 E^{\paren{\textbf{S}}}}{\partial\hat{K}_{a_1,b_1}\cdot\partial\hat{K}_{a_2,b_2}}
=&\frac{2 Q_{b_1} Q_{b_2}}{D\cdot T}\sum_{t=1}^T\left(\frac{\partial\hat{S}_t}{\partial\hat{A}_{a_1}}\cdot\frac{\partial\hat{S}_t}{\partial\hat{A}_{a_2}}\right.+\\
&\left.\paren{\hat{S}_t-S_t}\cdot\frac{\partial^2\hat{S}_t}{\partial\hat{A}_{a_1}\cdot\partial\hat{A}_{a_2}}\right)
\end{align*}

When $\hat{\textbf{K}}=\textbf{K}$, we get:
\begin{align*}
\left.\frac{\partial E^{\paren{\textbf{S}}}}{\partial\hat{K}_{a,b}}
\right\rvert_{\hat{\textbf{K}}=\textbf{K}}=&0\\
\left.\frac{\partial^2 E^{\paren{\textbf{S}}}}{\partial\hat{K}_{a_1,b_1}\cdot\partial\hat{K}_{a_2,b_2}}
\right\rvert_{\hat{\textbf{K}}=\textbf{K}}
=&\frac{2 Q_{b_1} Q_{b_2}}{D}\sum_{t=1}^T\paren{\frac{\partial S_t}{\partial A_{a_1}}\cdot\frac{\partial S_t}{\partial A_{a_2}}}
\end{align*}

Substituting them into Taylor expansion, we get:
\begin{align*}
&E^{\paren{\textbf{S}}}\\
\approx&\frac{1}{D\cdot T}\sum_{a_1=1}^T\sum_{b_1=1}^D\sum_{a_2=1}^T\sum_{b_2=1}^D\sum_{t=1}^T\\
&\paren{Q_{b_1}\cdot\frac{\partial\hat{S}_t}{\partial\hat{A}_{a_1}}\cdot\Delta K_{a_1,b_1}}
\paren{Q_{b_2}\cdot\frac{\partial\hat{S}_t}{\partial\hat{A}_{a_2}}\cdot\Delta K_{a_2,b_2}}
\end{align*}

Again, since we would like to equally divide the quantization error into every source \shichen{Need more argumentation}, we let the following equation hold for all $t=1,\cdots,T$, $a=1,\cdots,T$, and $b=1,\cdots,D$:
$$
E^{\paren{\textbf{S}}}_\text{max}\ge\frac{1}{D\cdot T}\cdot T\cdot D\cdot T\cdot D\cdot T\cdot\paren{Q_b\cdot\frac{\partial\hat{S}_t}{\partial\hat{A}_a}\cdot\Delta K_{a,b}}^2
$$

Therefore, we get:
$$
\Delta K_{a,b}\le\frac{\sqrt{E^{\paren{\textbf{S}}}_\text{max}}}{\sqrt{D}\cdot T}\cdot\frac{1}{\abs{Q_b\cdot\frac{\partial\hat{S}_t}{\partial\hat{A}_a}}}
$$
which is the same as:
$$
\Delta K_{t,i}\le\frac{\sqrt{E^{\paren{\textbf{S}}}_\text{max}}}{\sqrt{D}\cdot T}\cdot\frac{1}{\abs{Q_i\cdot\frac{\partial\hat{S}_j}{\partial\hat{A}_t}}}
$$

Finally, in order to bound $\Delta K_t$, we have:
\begin{align*}
\Delta K_t&\le\min_{i=1}^D\min_{j=1}^T\frac{\sqrt{E^{\paren{\textbf{S}}}_\text{max}}}{\sqrt{D}\cdot T}\cdot\frac{1}{\abs{Q_i\cdot\frac{\partial\hat{S}_j}{\partial\hat{A}_t}}}\\
&=\frac{\sqrt{E^{\paren{\textbf{S}}}_\text{max}}}{\sqrt{D}\cdot T}\cdot\frac{1}{\max_{i=1}^D\max_{j=1}^T\abs{Q_i\cdot\frac{\partial\hat{S}_j}{\partial\hat{A}_t}}}\\
&\le\frac{\sqrt{E^{\paren{\textbf{S}}}_\text{max}}}{\sqrt{D}\cdot T}\cdot\frac{1}{\max_{i=1}^D\abs{Q_i}\cdot\max_{j=1}^T\abs{\frac{\partial\hat{S}_j}{\partial\hat{A}_t}}}
\end{align*}

In the above formula, we can use the $\alpha$-th percentile of the query tensor as the estimation of $\max_{i=1}^D\abs{Q_i}$, which makes the inequality true with probability $\alpha\%$. As for $\max_{j=1}^T\abs{\frac{\partial\hat{S}_j}{\partial\hat{A}_t}}$, it can be calculated using the following equation:
$$
\frac{\partial\hat{S}_j}{\partial\hat{A}_t}
=\left\{\begin{aligned}
&S_j-S_j\cdot S_t,&\text{if } j=t\\
&-S_j\cdot S_t,&\text{if } j\neq t
\end{aligned}\right.
$$

\subsection{Step 3: distribution-aware quantization}

Since key cache and value cache are equivalent to each other in this step, we only demonstrate the process using key cache $\textbf{K}$.

For uniform quantization to $B^{\paren{\textbf{K}}}_t$ bits, we uniformly split the range $\left[K_t^\text{min},K_t^\text{max}\right]$ into $2^{B^{\paren{\textbf{K}}}_t}-1$ segments. So, the following inequality is hold:
$$
2\cdot\Delta K_t\cdot\paren{2^{B^{\paren{\textbf{K}}}_t}-1}\le K_t^\text{max}-K_t^\text{min}
$$

Therefore, we get:
$$
B^{\paren{\textbf{K}}}_t\ge\ceil{\log_2\paren{\frac{K_t^\text{max}-K_t^\text{min}}{2\cdot\Delta K_t}+1}}
$$

For normal quantization to $B^{\paren{\textbf{K}}}_t$ bits (for simplicity we use $b$ to denote $B^{\paren{\textbf{K}}}_t$ in the rest of this subsection), we assume that each entry in key cache follows the normal distribution $\mathcal{N}\paren{0,\sigma}$ and quantize all values in the range $\left[z_{\frac{i}{2^b}},z_{\frac{i+1}{2^b}}\right)$ to the quantization point $z_{\frac{i+0.5}{2^b}}$ for all $i=0,\cdots,2^b-1$, where $z_\alpha$ represents the $\alpha$-quantile of the distribution $\mathcal{N}\paren{0,\sigma}$. For a given $i$, the mean absolute error $\epsilon_i$ in the corresponding range can be calculated as:
\begin{align*}
\epsilon_i
&=2^b\int_{z_{\frac{i}{2^b}}}^{z_{\frac{i+1}{2^b}}}\abs{x-z_{\frac{i+0.5}{2^b}}}\cdot\frac{1}{\sqrt{2\pi}\sigma}e^{-\frac{x^2}{2\sigma^2}}\cdot\mathrm{d}x\\
&=\frac{2^b\cdot\sigma}{\sqrt{2\pi}}\paren{2\cdot\mathbf{E}\paren{i+0.5}-\mathbf{E}\paren{i}-\mathbf{E}\paren{i+1}}
\end{align*}
where $\mathbf{E}\paren{x}$ is defined as $e^{-\paren{\text{erfc}^{-1}\paren{\frac{x}{2^{b-1}}}}^2}$ and $\text{erfc}^{-1}\paren{\cdot}$ is the inversed complementary error function.

Averaging over all ranges, we get:
\begin{align*}
&\Delta K_t=\frac{1}{2^b}\sum_{i=0}^{2^b-1}\epsilon_i\\
=&\paren{\frac{1}{\sqrt{2\pi}}\sum_{i=0}^{2^b-1}\paren{2\cdot\mathbf{E}\paren{i+0.5}-\mathbf{E}\paren{i}-\mathbf{E}\paren{i+1}}}\cdot\sigma
\end{align*}

Note that $\Delta K_t$ is proportional to $\sigma$ and the coefficient is only related to $b$. Here are the calculated coefficients with the number of bits per token $b$ ranging from 1 to 8:
\begin{center}
    \begin{tabular}{cr}
        \toprule
        $B^{\paren{\textbf{K}}}_t$ & $\Delta K_t$ \\
        \midrule
        $1$ & $0.473222\cdot\sigma$\\
        $2$ & $0.271204\cdot\sigma$\\
        $3$ & $0.151629\cdot\sigma$\\
        $4$ & $0.0832674\cdot\sigma$\\
        $5$ & $0.0451210\cdot\sigma$\\
        $6$ & $0.0242022\cdot\sigma$\\
        $7$ & $0.0128782\cdot\sigma$\\
        $8$ & $0.00680873\cdot\sigma$\\
        \bottomrule
    \end{tabular}
\end{center}

Using the above table, we can choose the smallest $B^{\paren{\textbf{K}}}_t$ that satisfies the given requirement of maximum absolute error per token $\Delta K_t$.

